Uncertainty Modeling for Out-of-Distribution Generalization

Though remarkable progress has been achieved in various vision tasks, deep neural networks still suffer obvious performance degradation when tested in out-of-distribution scenarios. We argue that the feature statistics (mean and standard deviation), which carry the domain characteristics of the training data, can be properly manipulated to improve the generalization ability of deep learning models. Common methods often consider the feature statistics as deterministic values measured from the learned features and do not explicitly consider the uncertain statistics discrepancy caused by potential domain shifts during testing. In this paper, we improve the network generalization ability by modeling the uncertainty of domain shifts with synthesized feature statistics during training. Specifically, we hypothesize that the feature statistic, after considering the potential uncertainties, follows a multivariate Gaussian distribution. Hence, each feature statistic is no longer a deterministic value, but a probabilistic point with diverse distribution possibilities. With the uncertain feature statistics, the models can be trained to alleviate the domain perturbations and achieve better robustness against potential domain shifts. Our method can be readily integrated into networks without additional parameters. Extensive experiments demonstrate that our proposed method consistently improves the network generalization ability on multiple vision tasks, including image classification, semantic segmentation, and instance retrieval. The code can be available at https://github.com/lixiaotong97/DSU.

==> alg.tex <==
\usepackage{algpseudocode}
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[ruled,linesnumbered]{algorithm2e}

\begin{algorithm}[htp]
\small 
%\footnotesize
\caption{The overall training procedure}
\label{alg:algorithm1}
\KwIn{
Source labeled dataset $\{(x^{s}_{i},y^{s}_{i})\}$ and target unlabeled dataset $\{x^{t}_{i}\}$;
}
\KwOut{
The trained backbone network $f(\cdot)$ and classifier $\varphi(\cdot)$;
}
    
Initialize the backbone network $f(\cdot)$ with the ImageNet-pretrained ResNet-50;

Initialize the XBM memory as an empty queue $M$;

Plug our IDM module after the $m$-th stage of the backbone $f(\cdot)$ and randomly initialize it.

\For{$epoch=1$ to MaxEpochs}
{
Use the backbone $f(\cdot)$ to extract features $\{f^{t}_{i}\}$ for the target dataset $\{x^{t}_{i}\}$;

Assign pseudo labels $\{y^{t}_{i}\}$ for target domain samples $\{x^{t}_{i}\}$ by performing DBSCAN clustering on the target features $\{f^{t}_{i}\}$;

\For{$iter=1$ to MaxIters}
{

Sample a mini-batch of samples including $n$ source samples $\{(x^{s}_{i},y^{s}_{i})\}_{i=1}^{n}$ and $n$ target samples $\{(x^{t}_{i},y^{t}_{i})\}_{i=1}^{n}$;

Feed forward the batch into the network to obtain the features and predictions for the source, target, and intermediate domains: $(f^{s},\varphi^{s})$, $(f^{t},\varphi^{t})$, and $(f^{\rm inter},\varphi^{\rm inter})$;

\If {using XBM}{

Enqueue($M$, $\{(f^{t},y^{t})\}$, $\{(f^{s},y^{s})\}$);

\If {M is full}{
Dequeue($M$);
}
Use all entries in $M$ for the hard negatives mining in the triplet loss in $\mathcal L_{\rm ReID}$ from Eq.~(\textcolor{red}{9});

}


Calculate the overall training loss by Eq. (\textcolor{red}{9});

Update $f(\cdot)$, $\varphi(\cdot)$, and our IDM module together by back-propagating the gradients of Eq. (\textcolor{red}{9});
}
}
\end{algorithm}
